Dynamic Transformers Provide a False Sense of Efficiency

Despite much success in natural language processing (NLP), pre-trained language models typically lead to a high computational cost during inference. Multi-exit is a mainstream approach to address this issue by making a trade-off between efficiency and accuracy, where the saving of computation comes from an early exit. However, whether such saving from early-exiting is robust remains unknown. Motivated by this, we first show that directly adapting existing adversarial attack approaches targeting model accuracy cannot significantly reduce inference efficiency. To this end, we propose a simple yet effective attacking framework, SAME, a novel slowdown attack framework on multi-exit models, which is specially tailored to reduce the efficiency of the multi-exit models. By leveraging the multi-exit models' design characteristics, we utilize all internal predictions to guide the adversarial sample generation instead of merely considering the final prediction. Experiments on the GLUE benchmark show that SAME can effectively diminish the efficiency gain of various multi-exit models by 80% on average, convincingly validating its effectiveness and generalization ability.

==> Approach/alg.tex <==
\subsection{Attack Algorithm}
The attack algorithm is shown as Algorithm~\ref{alg:algorithm}. 
Our attack algorithm accepts three inputs: a benign input text $x$, the victim dynamic multi-exit language model $\mathcal{F}$, and the maximum iteration number $T$. Our algorithm outputs an adversarial example $x_{adv}$ that satisfies the constraints specified in Eq.~\ref{eq:problem}. 
In the algorithm, we initialize the adversarial example as the benign input text $x$ and the mutant seed set $\mathcal{G}$. After that, we iteratively update the best adversarial example $x_{adv}$. Specifically, we compute the uniform loss based on Eq.~\ref{eq:uniform} and the heuristic loss based on Eq.~\ref{eq:heuritic}. We then get the gradient by the losses (Eq.~\ref{eq:weight_loss}). In the end, we adopt the classic beam search approach to complete the query-based attack.



\begin{algorithm}[t!]
\caption{ \tool Attacking Framework}
\label{alg:algorithm}
{\bf Require:}
Benign Text $ x $; pre-trained dynamic multi-exit language model $ \mathcal{F}$; iterations $ T $. \\
{\bf Ensure:}
Optimal adversarial example $ x_{adv} $.\\
$ x_{adv} = x $;\\
$ \mathcal{G} = \{\emptyset\} $ $\vartriangleleft$ Initialize 
the mutant seed set \\
\For{each $ t\in T $}
{
    Calculate uniform loss by Eq.~\ref{eq:uniform} \\
    Calculate heuristic loss by Eq.~\ref{eq:heuritic} \\
    Calculate energy loss by Eq.~\ref{eq:weight_loss} \\
    Generate gradients $grad$ by energy loss \\
    $\mathcal{G'} = \{\emptyset\} $ $\vartriangleleft$ Initialize an empty set\\ 
    \For{each token $\in$ $x_a$}
    {
        Generate a mutant $x'$ based on $grad$ \\
        $\mathcal{G} = \mathcal{G} \cup x' $ $\vartriangleleft$ add the mutant to set\\
    }
    Select candidates $\mathcal{G'}$ by beam search \\
    Update best adversary $x_{adv}$ by $\mathcal{G'}$ \\
    Update mutant seed set $\mathcal{G}$ by $\mathcal{G'}$ \\
}
\Return{$x_{adv}$}
\end{algorithm}
